Communication and Storage Efficient Federated Split Learning

Federated learning (FL) is a popular distributed machine learning (ML) paradigm, but is often limited by significant communication costs and edge device computation capabilities. Federated Split Learning (FSL) preserves the parallel model training principle of FL, with a reduced device computation requirement thanks to splitting the ML model between the server and clients. However, FSL still incurs very high communication overhead due to transmitting the smashed data and gradients between the clients and the server in each global round. Furthermore, the server has to maintain separate models for every client, resulting in a significant computation and storage requirement that grows linearly with the number of clients. This paper tries to solve these two issues by proposing a communication and storage efficient federated and split learning (CSE-FSL) strategy, which utilizes an auxiliary network to locally update the client models while keeping only a single model at the server, hence avoiding the communication of gradients from the server and greatly reducing the server resource requirement. Communication cost is further reduced by only sending the smashed data in selected epochs from the clients. We provide a rigorous theoretical analysis of CSE-FSL that guarantees its convergence for non-convex loss functions. Extensive experimental results demonstrate that CSE-FSL has a significant communication reduction over existing FSL techniques while achieving state-of-the-art convergence and model accuracy, using several real-world FL tasks.

==> related-work.tex <==
Compared with FL, SL \cite{gupta2018distributed} enables learning on resource-constrained clients by splitting the neural network model into two parts and keeping only the first few layers on the client. Variants of SL have been proposed to handle different tasks, such as in the healthcare domain \cite{vepakomma2018split, abuadbba2020can, poirot2019split}, privacy \cite{kim2020multiple} or for IoT devices \cite{matsubara2021neural, palanisamy2021spliteasy, gao2020end}. However, the current client needs to wait for the completion of the previous client training before its own training, which is not efficient. 

By combining the advantages of FL and SL, SplitFed \cite{thapa2020splitfed} achieves model training in an SL setup with multiple clients training in parallel as in FL. Although the FSL method can improve the efficiency of client-side model training compared with SL, it still suffers from large communication costs. For each mini-batch data, the server would receive smashed data from all participating clients to train the server-side model, and all participating clients need to wait to receive gradients from the server to update their own models. As a result, the communication overhead for both upstream and downstream is significant. A local-loss-based training with SL is proposed in \cite{han2021accelerating}, which reduces the downstream load by updating the client-side locally via introducing the auxiliary network. Nonetheless, it still requires huge storage space at the server to keep multiple copies of server-side model updates, one per client. Besides, the previous works do not consider upstream communication cost. 

Inspired by these limitations, our work focuses on designing a communication and storage efficient FSL method to reduce the communication load for both upstream and downstream, while keeping only one server-side model to save storage.
